Pairwise Fairness for Ranking and Regression

We present pairwise fairness metrics for ranking models and regression models that form analogues of statistical fairness notions such as equal opportunity, equal accuracy, and statistical parity. Our pairwise formulation supports both discrete protected groups, and continuous protected attributes. We show that the resulting training problems can be efficiently and effectively solved using existing constrained optimization and robust optimization techniques developed for fair classification. Experiments illustrate the broad applicability and trade-offs of these methods.

==> figures/tab-business.tex <==
\begin{figure*}[h]
\footnotesize
\begin{subfigure}[t]{0.45\textwidth}
\centering
\begin{tabular}{c|ccc|c}
    %
    & \textbf{Chain} & \textbf{Non-chain} \\
    %
    \hline
    %
    \textbf{Row-avg} &    0.767 &    0.706\\
    \hline
    %
    %
\end{tabular}
\caption{Unconstrained}
\end{subfigure}
%
\begin{subfigure}[t]{0.45\textwidth}
\centering
\begin{tabular}{c|ccc|c}
    %
    & \textbf{Chain} & \textbf{Non-chain} \\
    %
    \hline
    %
    \textbf{Row-avg} &    0.780 &    0.719\\
    \hline
    %
    %
\end{tabular}
\caption{Debiased}
\end{subfigure}
%
\\
\begin{subfigure}[t]{0.45\textwidth}
\centering
\begin{tabular}{c|ccc|c}
    %
    & \textbf{Chain} & \textbf{Non-chain} \\
    %
    \hline
    %
    \textbf{Row-avg} &    {0.715} &    {0.712}\\
    \hline
    %
    %
\end{tabular}
\caption{Constrained}
\end{subfigure}
%
\begin{subfigure}[t]{0.45\textwidth}
\centering
\begin{tabular}{c|ccc|c}
    %
    & \textbf{Chain} & \textbf{Non-chain} \\
    %
    \hline
    %
    \textbf{Row-avg} &    
    {0.804} &    0.733\\
    \hline
    %
    %
\end{tabular}
\caption{Robust}
\end{subfigure}
%
\caption{Test row-based matrix averages on business match (ranking) data.}
\label{fig:business}
\end{figure*}

==> figures/tab-experts-ranking.tex <==
\begin{figure*}[h!]
\begin{subfigure}[t]{0.48\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1.1cm}\textbf{Non-expert} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Expert}} 
  \hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Male} & \textbf{Female} \\
    %
    \hline
    %
    \textbf{Male}   &  0.534 &   0.028 \\
    \textbf{Female} &  0.991 &   0.573 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Unconstrained}
\end{subfigure}
%
\begin{subfigure}[t]{0.48\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1.1cm}\textbf{Non-expert} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Expert}} \hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Male} & \textbf{Female} \\
    %
    \hline
    %
    \textbf{Male}   &  0.541 &   0.081 \\
    \textbf{Female} &  0.977 &   0.571 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Debiased}
\end{subfigure}
% 
\\
\begin{subfigure}[t]{0.48\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1.1cm}\textbf{Non-expert} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Expert}} \hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Male} & \textbf{Female} \\
    %
    \hline
    %
    \textbf{Male}   &  0.540 &   {0.501} \\
    \textbf{Female} &  {0.601} &   0.571 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Constrained/Cross-groups}
\end{subfigure}
%
\begin{subfigure}[t]{0.48\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1.1cm}\textbf{Non-expert} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Expert}} \hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Male} & \textbf{Female} \\
    %
    \hline
    %
    Male   &  0.540 &   {0.471} \\
    Female &  {0.614} &   0.553 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Robust/Cross-groups}
\end{subfigure}
%
\vspace{-5pt}
\caption{Test pairwise accuracy matrix for W3C experts (ranking) data.}
\label{fig:matrix-experts}
\end{figure*}

==> figures/tab-matrix.tex <==
\begin{table}[H] 

\centering

\caption{Example group-dependent pairwise accuracy matrix of $K=3$ groups, and the frequency-weighted row mean and column mean for the restaurant ranking example in the introduction.}

\label{tab:matrix}
\small
\begin{tabular}{cc}
  %
  & \textbf{Expensive} \\[5pt]
  %
  \hspace{-15pt}\rotatebox[origin=c]{90}{\textbf{Cheap}}
 \hspace{-15pt}	  
   &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{French} & \textbf{Mexican} & \textbf{Chinese} & \textbf{Row Mean} \\
    %
    \hline
    %
    \textbf{French} & \textit{0.76} & 0.68 & 0.56 & 0.70 \\
    \textbf{Mexican} & 0.61 & \textit{0.62} & 0.55 & 0.60 \\
    \textbf{Chinese} & 0.62 & 0.61 & \textit{0.56} & 0.60 \\
    %
    \hline
    %
    \textbf{Col.\ Mean} & 0.69 & 0.65 & 0.56 & \textit{0.65}
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}

\end{table}


==> figures/tab-regression.tex <==
%\begin{figure}[t]
%%%
\begin{figure}[h!]
\footnotesize
\begin{subfigure}[t]{0.46\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1cm} \textbf{Low} \\
  %
  \rotatebox[origin=c]{90}{\textbf{High}}\hspace{-10pt}  &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Male} & \textbf{Female} \\
    %
    \hline
    %
    Male   &  0.653 &   0.490 \\
    Female &  0.795 &   0.654 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Unconstrained}
\end{subfigure}
%
\begin{subfigure}[t]{0.46\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1cm} \textbf{Low} \\
  %
  \rotatebox[origin=c]{90}{\textbf{High}} \hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Male} & \textbf{Female} \\
    %
    \hline
    %
    \textbf{Male}   &  0.652 &   {0.647} \\
    \textbf{Female} &  {0.666} &   0.655 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Constrained/Cross-groups}
\end{subfigure}
%
\caption{Pairwise accuracy matrix for law school (regression).}
\label{fig:law}
\end{figure}
%
%
% \begin{figure}[t]
% \footnotesize
% \begin{subfigure}[t]{0.23\textwidth}
% \begin{tabular}{cc}
%   %
%   & \hspace{1cm} \textbf{Low} \\
%   %
%   \rotatebox[origin=c]{90}{\textbf{High}}\hspace{-10pt}  &
%   %
%   \begin{tabular}{c|ccc|c}
%     %
%     & \textbf{$\cacc{>}$} & \textbf{$\cacc{<}$} \\
%     %
%     \hline
%     %
%     Other &  0.742 &  0.462 \\
%     Black &  0.944 &  0.782 \\
%     \hline
%     %
%     %
%   \end{tabular}
%   %
%   \\
%   %
% \end{tabular}
% \caption{Unconstrained}
% \end{subfigure}
% %
% \begin{subfigure}[t]{0.23\textwidth}
% \begin{tabular}{cc}
%   %
%   & \hspace{1cm} \textbf{Low} \\
%   %
%   \rotatebox[origin=c]{90}{\textbf{High}}\hspace{-10pt}  &
%   %
%   \begin{tabular}{c|ccc|c}
%     %
%     & \textbf{Other} & \textbf{Black} \\
%     %
%     \hline
%     %
%     Other &  \textbf{\textit{0.678}} &  \textbf{0.733} \\
%     Black &  \textbf{0.687} &  \textbf{\textit{0.739}} \\
%     \hline
%     %
%     %
%   \end{tabular}
%   %
%   \\
%   %
% \end{tabular}
% \caption{Constrained/All}
% \end{subfigure}
% %
% \vspace{-5pt}
% \caption{Pairwise accuracy matrix for crime (regression) data.}
% \label{fig:crime-regression}
% \vspace{-10pt}
% \end{figure}
%\end{figure}
%
%
\begin{figure}[H]
\footnotesize
\begin{subfigure}[t]{0.46\textwidth}
\centering
\begin{tabular}{cc}
    %
    $\cacc{>}$ & $\cacc{<}$ \\
    %
    \hline
    %
    %\textbf{Row-avg} &    
    0.904 & 0.577
    \\
    \hline
    %
    %
\end{tabular}
\caption{Unconstrained}
\end{subfigure}
\begin{subfigure}[t]{0.46\textwidth}
\centering
\begin{tabular}{cc}
    %
    $\cacc{>}$ & $\cacc{<}$ \\
    %
    \hline
    %
    %\textbf{Row-avg} &    
    {0.777} & {0.745}
    \\
    \hline
    %
    %
\end{tabular}
\caption{Constrained/Continuous Attr.}
\end{subfigure}
\caption{Continuous attribute pairwise accuracies for crime (regression) with \%.\ of black population as protected attribute.}
\label{fig:crime-regression}
%\vspace{10cm}
\end{figure}

==> figures/tab-simulated-full.tex <==
\begin{figure*}[h!]
\footnotesize
\begin{subfigure}[t]{0.32\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1.2cm}\textbf{Negative} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Positive}} \hspace{-10pt} &
  %
  \begin{tabular}{c|cc}
    %
    & \textbf{$G_0$} & \textbf{$G_1$} \\
    %
    \hline
    %
    \textbf{$G_0$} &    0.941 &    0.980 \\
    \textbf{$G_1$} &    0.705 &    0.894 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Unconstrained}
\end{subfigure}
%
\begin{subfigure}[t]{0.32\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1.2cm}\textbf{Negative} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Positive}} \hspace{-10pt}
  &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{$G_0$} & \textbf{$G_1$} \\
    %
    \hline
    %
    \textbf{$G_0$} &    {0.743} &    {0.769} \\
    \textbf{$G_1$} &    {0.779} &    {0.797} \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Constrained}
\end{subfigure}
%
\begin{subfigure}[t]{0.32\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1.2cm}\textbf{Negative} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Positive}}
  \hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{$G_0$} & \textbf{$G_1$} \\
    %
    \hline
    %
    \textbf{$G_0$ } &    {{0.881}} &    0.930 \\
    \textbf{$G_1$} &    0.897 &    0.935 \\
    \hline
    %
    %
  \end{tabular}
  %
  %
\end{tabular}
\caption{Robust}
\end{subfigure}
\caption{Test pairwise accuracy matrix for simulated (ranking) data two groups, with both cross-group and in-group criteria.}
\label{fig:matrix-simulated}
\vspace{-5pt}
\end{figure*}

==> figures/tab-simulated.tex <==
\begin{figure*}
\begin{subfigure}[t]{0.25\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1.2cm}\textbf{Negative} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Positive}} \hspace{-10pt} &
  %
  \begin{tabular}{c|cc}
    %
    & \textbf{$G_0$} & \textbf{$G_1$} \\
    %
    \hline
    %
    \textbf{$G_0$} &    0.941 &    0.980 \\
    \textbf{$G_1$} &    0.705 &    0.894 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Sim./Unconstrained}
\end{subfigure}
%
\begin{subfigure}[t]{0.25\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1.2cm}\textbf{Negative} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Positive}} \hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{$G_0$} & \textbf{$G_1$} \\
    %
    \hline
    %
    \textbf{$G_0$} &    0.854 &   { 0.900} \\
    \textbf{$G_1$} &    {0.907} &    0.927 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Sim./Constrained}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
\centering
\begin{tabular}{ccc}
    %
    \textbf{$G_0$} & \textbf{$G_1$} & \textbf{$G_2$} \\
    %
    \hline
    %
    %  0.779 &  0.759 &  0.779\\
    % 0.710 &  0.700  &  0.728\\
    0.714 & 0.699 & 0.729\\
    \hline
    %
    %
\end{tabular}
\caption{Sim./Constrained}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\textwidth}
\centering
\begin{tabular}{ccc}
    %
     \textbf{$G_0$} & \textbf{$G_1$} & \textbf{$G_2$} \\
    %
    \hline
    %
    %   0.930 &  0.879 & 0.885\\
    0.881 & 0.877 & 0.949\\
    \hline
    %
    %
\end{tabular}
\caption{Sim./Robust}
\end{subfigure}
% \begin{subfigure}[t]{0.18\textwidth}
% \centering
% \begin{tabular}{cc}
%     %
%     \textbf{C} & \textbf{NC} \\
%     %
%     \hline
%     %
%      0.767 &    0.706\\
%     \hline
%     %
%     %
% \end{tabular}
% \caption{Business/Uncons.}
% \end{subfigure}
% %
% \begin{subfigure}[t]{0.17\textwidth}
% \centering
% \begin{tabular}{cc}
%     %
%      \textbf{C} & \textbf{NC} \\
%     %
%     \hline
%     %
%       {0.715} &    {0.712}\\
%     \hline
%     %
%     %
% \end{tabular}
% \caption{Business/Constr.}
% \end{subfigure}
% \begin{subfigure}[t]{0.18\textwidth}
% \centering
% \begin{tabular}{cc}
%     %
%      \textbf{C} & \textbf{NC} \\
%     %
%     \hline
%     %
%       {0.804} &    0.733\\
%     \hline
%     %
%     %
% \end{tabular}
% \caption{Business/Robust}
% \end{subfigure}
%
\\[3pt]
\begin{subfigure}[t]{0.32\textwidth}
\centering
\begin{tabular}{cc}
  %
  &\hspace{0.9cm} \textbf{Non-toxic} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Toxic}}\hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Other} & \textbf{Gay} \\
    %
    \hline
    %
    \textbf{Other} &  0.973 &  0.882 \\
    \textbf{Gay}   &  0.986 &  0.937 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Wiki/Unconst.}
\end{subfigure}
%
\begin{subfigure}[t]{0.32\textwidth}
\centering
\begin{tabular}{cc}
  %
  &\hspace{0.9cm} \textbf{Non-toxic} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Toxic}}\hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Other} & \textbf{Gay} \\
    %
    \hline
    %
    \textbf{Other} &  0.971 &  {0.953} \\
    \textbf{Gay}   &  {0.967} &  0.945 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Wiki/Debiased}
\end{subfigure}
%
\begin{subfigure}[t]{0.32\textwidth}
\centering
\begin{tabular}{cc}
  %
  &\hspace{0.9cm} \textbf{Non-toxic} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Toxic}}\hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Other} & \textbf{Gay} \\
    %
    \hline
    %
    \textbf{Other} &  0.962 &  {0.943} \\
    \textbf{Gay}   &  {0.953} &  0.922 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Wiki/Constrained}
\end{subfigure}
\vspace{-4pt}
%\caption{Test pairwise accuracy matrices for  Simulated ranking (a)--(b),  row-based matrix averages $\pacc{chain}{:}$  and $\pacc{non-chain}{:}$ for Business matching (c)--(e), and pairwise accuracy matrices for Wiki Talk Pages ranking (f)--(h).}
\caption{Test pairwise accuracy matrices for  Simulated ranking with 2 groups (a)--(b),  row-based matrix averages $\pacc{0}{:}$, $\pacc{1}{:}$ and $\pacc{2}{:}$ for Simulated ranking with 3 groups (c)--(d), and pairwise accuracy matrices for Wiki Talk Pages ranking (e)--(g).}
\label{fig:matrix-sim-law}
\vspace{-1pt}
\end{figure*}

==> figures/tab-summary-regression.tex <==
%%%
\begin{table*}
\begin{minipage}[t]{0.65\textwidth}
    \centering
    % \begin{tabular}{c|c|c|c|c|c|c|c}
    \begin{tabular}{lcccc}
        \hline
        \textbf{Dataset} & 
        \textbf{Prot. Group} &
        % \textbf{Problem} &
        %\textbf{Constraint Type} &  
        \textbf{Unconstrained} &
        \textbf{Beutel et al.} &
        \textbf{Constrained}  \\
        \hline
        %
        Law &
        %
        \textit{Gender} &
        %Cross-group &
        \textbf{0.142} ~(0.30) &
        0.167 ~(0.06) &
        \hlgt{0.143 ~(\textbf{0.02})}
        \\
        %
        % \multirow{2}{*}{Crime} &
        Crime &
        % \multirow{2}{*}{\textit{Race} (binary)} &
        % \textit{Race} &
        % \textbf{0.021}~(0.518) &
        % -- &
        % 0.098~(\textbf{0.019}) &
        % -- 
        % %
        % %
        % &
        % &
        % &
        % &
        % Cross-group  \& In-group &
        % \textbf{0.021} ~(0.483) &
        % 0.047 ~(\textbf{0.061}) 
        % \\
        \textit{Race \%} &
       % Cont.\ Attr.\ &
        \textbf{0.021} ~(0.33) &
        0.033 ~(\textbf{0.02}) &
        0.028 ~({0.03}) 
        %
        \\
        \hline
    \end{tabular}
    %\label{tab:results-summary-regression}
    % \vspace{-14pt}
\end{minipage}
\begin{minipage}[t]{0.34\textwidth}
\centering
\begin{tabular}{cc}
  %
  & \hspace{1cm} \textbf{Low} \\
  %
  \rotatebox[origin=c]{90}{\textbf{High}} \hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Male} & \textbf{Female} \\
    %
    \hline
    %
    \textbf{Male}   &  0.652 &   {0.647} \\
    \textbf{Female} &  {0.666} &   0.655 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\end{minipage}
\caption{Left: Regression test MSE (lower is better) and pairwise fairness violation (in parenthesis), with \hlgt{blue} indicating strictly best between last two columns. Right: Test pairwise accuracy matrix for \textit{constrained} optimization on Law School dataset. }
\label{tab:results-summary-regression}
\vspace{-10pt}
\end{table*}
%%%

==> figures/tab-summary.tex <==
%%%
\begin{table*}
    \centering
    % \begin{tabular}{c|c|c|c|c|c|c|c}
    \begin{tabular}{c|c|c|c|c|c|c}
        \hline
        \hline
        \textbf{Dataset} & 
        \textbf{Prot. Group} &
        % \textbf{Problem} &
        \textbf{Constraint Type} &  
        \textbf{Unconstrained} &
        \textbf{Debiased} &
        \textbf{Constrained} &  
        \textbf{Robust} \\
        \hline
        %
        \multirow{2}{*}{Simulated} &
        \multirow{2}{*}{0/1} &
        % \multirow{2}{*}{Ranking} &
        Cross-group &
        \textbf{0.919} ~(0.275) &
        \textbf{0.919} ~(0.275) &
        0.864 ~(\textbf{0.008}) &
        0.857 ~(0.018) 
        \\
        %
        &
        &
        % &
        Cross-group \& In-group &
        \textbf{0.919} ~(0.275) &
        \textbf{0.919} ~(0.275) &
        0.750 ~({0.054}) &
        {0.888} ~(\textbf{0.053}) 
        \\
        \hline
        %
        Business Matching &
        \textit{Business Type} &
        % Ranking &
        Marginal &
        \textbf{0.695} ~(0.062) &
        0.698 ~(0.061) &
        0.685 ~(\textbf{0.003}) &
        0.685 ~(0.071) 
        %
        \\
        \hline
        %
        Wiki Talk Page &
        %
        \textit{Term ``Gay''} &
        % Ranking &
        Cross-group &
        \textbf{0.974} ~(0.104) &
        0.972 ~(0.014) &
        0.962 ~(\textbf{0.010}) &
        0.941 ~(0.025)
        \\
        \hline
         %
        W3C Experts &
        %
        \textit{Gender} &
        % Ranking &
        Cross-group &
        {0.528} ~(0.963) &
        0.539 ~(0.895) &
        \textbf{0.544} ~(\textbf{0.100}) &
        0.542 ~(0.143) 
        \\
        \hline
        %
        Crime &
        %
        \textit{Race Percentage} &
        % Ranking &
        Continuous Attr. &
        \textbf{0.931} ~(0.184) &
        -- &
        0.810 ~(\textbf{0.036}) &
        {0.858} ~(\textbf{0.036}) 
    %     \hline
    %     %
    %     Law School &
    %     %
    %     \textit{Gender} &
    %     Regression &
    %     Off-diagonals &
    %   \textbf{0.140} ~(0.360) &
    %     -- &
    %     0.145 ~(\textbf{0.028}) &
    %     --
    %     \\
    %     \hline
    %     %
    %     % \multirow{2}{*}{Crime} &
    %     Crime &
    %     % \multirow{2}{*}{\textit{Race} (binary)} &
    %     \textit{Race} (binary) &
    %     %\multirow{2}{*}{Regression} &
    %     Regression &
    %     % Off-diagonals &
    %     % \textbf{0.021}~(0.518) &
    %     % -- &
    %     % 0.098~(\textbf{0.019}) &
    %     % -- 
    %     % %
    %     % %
    %     % &
    %     % &
    %     % &
    %     % &
    %     All &
    %     \textbf{0.021}~(0.518) &
    %     -- &
    %     0.104~(\textbf{0.018}) &
    %     -- 
    %     %
    %     \\
        \\
        \hline
        \hline
    \end{tabular}
    \caption{Test AUC with test pairwise fairness violations in parentheses. For fairness violations, we report $|\pacc{G_0}{G_1} - \pacc{G_1}{G_0}|$ when imposing cross-group constraints, 
    $\max\{|\pacc{G_0}{G_1} - \pacc{G_1}{G_0}|,~ |\pacc{G_0}{G_0} - \pacc{G_1}{G_1}|\}$ when imposing both cross-group and in-group constraints, $|\pacc{G_0}{:} - \pacc{G_1}{:}|$
    for marginal constraints,  and $|\cacc{>} - \cacc{<}|$ for the constraint on continuous protected attributes.
    }
    \label{tab:results-summary}
\vspace{-12pt}
\end{table*}
%%%

==> figures/tab-wiki-toxicity.tex <==

\begin{figure*}[h]
\footnotesize
\begin{subfigure}[t]{0.32\textwidth}
\centering
\begin{tabular}{cc}
  %
  &\hspace{0.9cm} \textbf{Non-toxic} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Toxic}}\hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Other} & \textbf{Gay} \\
    %
    \hline
    %
    \textbf{Other} &  0.973 &  0.882 \\
    \textbf{Gay}   &  0.986 &  0.937 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Unconstrained}
\end{subfigure}
%
\begin{subfigure}[t]{0.32\textwidth}
\centering
\begin{tabular}{cc}
  %
  &\hspace{0.9cm} \textbf{Non-toxic} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Toxic}}\hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Other} & \textbf{Gay} \\
    %
    \hline
    %
    \textbf{Other} &  0.971 &  \textbf{0.953} \\
    \textbf{Gay}   &  \textbf{0.967} &  0.945 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Debiased}
\end{subfigure}
%
\begin{subfigure}[t]{0.32\textwidth}
\centering
\begin{tabular}{cc}
  %
  &\hspace{0.9cm} \textbf{Non-toxic} \\
  %
  \rotatebox[origin=c]{90}{\textbf{Toxic}}\hspace{-10pt} &
  %
  \begin{tabular}{c|ccc|c}
    %
    & \textbf{Other} & \textbf{Gay} \\
    %
    \hline
    %
    \textbf{Other} &  0.962 &  \textbf{0.943} \\
    \textbf{Gay}   &  \textbf{0.953} &  0.922 \\
    \hline
    %
    %
  \end{tabular}
  %
  \\
  %
\end{tabular}
\caption{Constrained}
\end{subfigure}
% %
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \begin{tabular}{cc}
%   %
%   &\hspace{0.9cm} \textbf{Non-toxic} \\
%   %
%   \rotatebox[origin=c]{90}{\textbf{Toxic}}\hspace{-10pt} &
%   %
%   \begin{tabular}{c|ccc|c}
%     %
%     & \textbf{Other} & \textbf{Gay} \\
%     %
%     \hline
%     %
%     \textbf{Other} &  0.940 &  \textbf{0.920} \\
%     \textbf{Gay}   &  \textbf{0.945} &  0.927 \\
%     \hline
%     %
%     %
%   \end{tabular}
%   %
%   \\
%   %
% \end{tabular}
% \caption{Robust/Cross-groups}
% \end{subfigure}
\vspace{-5pt}
\caption{Test pairwise accuracy matrix on Wiki Talk Page comments (ranking) data.}
\vspace{-5pt}
\label{fig:wiki}
\end{figure*}
%%%

==> helpers.tex <==
\usepackage{amsfonts}  % blackboard math symbols
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{appendix}
\usepackage{bbold}
\usepackage{booktabs}  % professional-quality tables
\usepackage{color}
\usepackage{courier}
\usepackage{float}
\usepackage{graphicx}
\usepackage{helvet}
\usepackage{mathtools}
\usepackage{mdwlist}  % single-spaced itemize* and enumerate*
\usepackage{microtype}  % microtypography
\usepackage{multirow}
\usepackage{natbib}
\usepackage{nicefrac}  % compact symbols for 1/2, etc.
% \usepackage{subfigure}
\usepackage[T1]{fontenc}  % use 8-bit T1 fonts
\usepackage{tabularx}
\usepackage{times}
\usepackage{url}  % simple URL typesetting
\usepackage[utf8]{inputenc}  % allow utf-8 input
\usepackage{verbatim}
\usepackage{wrapfig}
\usepackage{xspace}

\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{hyperref}  % hyperlinks


%%
\usepackage{subcaption}
%%

% Use symbols for footnotes, so that they don't look like exponents when they're
% attached to equations.
%\renewcommand*{\thefootnote}{\fnsymbol{footnote}}

% turn off boxes around links
\hypersetup{colorlinks = false, pdfborder = {0 0 0}}

% make it less likely that text will encroach into the margins
\setlength{\emergencystretch}{3em}

% defining the \BibTeX command - from Oren Patashnik's original BibTeX documentation.
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08emT\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% TODO and NOTE macros.
\newif\ifdraft
%\draftfalse
\drafttrue
\newcommand{\TODO}[1]{
  \ifdraft
    \textcolor{red}{[TODO: #1]}\xspace
  \fi
}
\newcommand{\NOTE}[1]{
  \ifdraft
    \textcolor{blue}{[NOTE: #1]}\xspace
  \fi
}

% How we refer to Google in the paper, depending on whether or not it's
% accepted.
\ifdefined\isaccepted
  \newcommand{\google}{Google\xspace}
  \newcommand{\Google}{Google\xspace}
\else
  \newcommand{\google}{a large internet services company\xspace}
  \newcommand{\Google}{A large internet services company\xspace}
\fi

% paragraph spacing
\renewcommand{\paragraph}[1]{\textbf{#1}\;\xspace}
% plot size
\newcommand{\plotwidth}{0.47\textwidth}

% References to various items
%\renewcommand{\eqref}[1]{Equation~\ref{eq:#1}}
\renewcommand{\eqref}[1]{(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\algref}[1]{Algorithm~\ref{alg:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\facref}[1]{Fact~\ref{fac:#1}}
\newcommand{\itemref}[1]{Item~\ref{item:#1}}
% References to two items at a time
%\newcommand{\eqrefs}[3][and]{Equations~\ref{eq:#2} #1~\ref{eq:#3}}
\newcommand{\eqrefs}[3][and]{(\ref{eq:#2}) #1~(\ref{eq:#3})}
\newcommand{\secrefs}[3][and]{Sections~\ref{sec:#2} #1~\ref{sec:#3}}
\newcommand{\apprefs}[3][and]{Appendices~\ref{app:#2} #1~\ref{app:#3}}
\newcommand{\figrefs}[3][and]{Figures~\ref{fig:#2} #1~\ref{fig:#3}}
\newcommand{\tabrefs}[3][and]{Tables~\ref{tab:#2} #1~\ref{tab:#3}}
\newcommand{\algrefs}[3][and]{Algorithms~\ref{alg:#2} #1~\ref{alg:#3}}
\newcommand{\thmrefs}[3][and]{Theorems~\ref{thm:#2} #1~\ref{thm:#3}}
\newcommand{\lemrefs}[3][and]{Lemmas~\ref{lem:#2} #1~\ref{lem:#3}}
\newcommand{\correfs}[3][and]{Corollaries~\ref{cor:#2} #1~\ref{cor:#3}}
\newcommand{\defrefs}[3][and]{Definitions~\ref{def:#2} #1~\ref{def:#3}}
\newcommand{\facrefs}[3][and]{Facts~\ref{fac:#2} #1~\ref{fac:#3}}
\newcommand{\itemrefs}[3][and]{Items~\ref{item:#2} #1~\ref{item:#3}}
% References to three items at a time
%\newcommand{\eqrefss}[4][and]{Equations~\ref{eq:#2}, \ref{eq:#3} #1~\ref{eq:#4}}
\newcommand{\eqrefss}[4][and]{(\ref{eq:#2}), (\ref{eq:#3}) #1~(\ref{eq:#4})}
\newcommand{\secrefss}[4][and]{Sections~\ref{sec:#2}, \ref{sec:#3} #1~\ref{sec:#4}}
\newcommand{\apprefss}[4][and]{Appendices~\ref{app:#2}, \ref{app:#3} #1~\ref{app:#4}}
\newcommand{\figrefss}[4][and]{Figures~\ref{fig:#2}, \ref{fig:#3} #1~\ref{fig:#4}}
\newcommand{\tabrefss}[4][and]{Tables~\ref{tab:#2}, \ref{tab:#3} #1~\ref{tab:#4}}
\newcommand{\algrefss}[4][and]{Algorithms~\ref{alg:#2}, \ref{alg:#3} #1~\ref{alg:#4}}
\newcommand{\thmrefss}[4][and]{Theorems~\ref{thm:#2}, \ref{thm:#3} #1~\ref{thm:#4}}
\newcommand{\lemrefss}[4][and]{Lemmas~\ref{lem:#2}, \ref{lem:#3} #1~\ref{lem:#4}}
\newcommand{\correfss}[4][and]{Corollaries~\ref{cor:#2}, \ref{cor:#3} #1~\ref{cor:#4}}
\newcommand{\defrefss}[4][and]{Definitions~\ref{def:#2}, \ref{def:#3} #1~\ref{def:#4}}
\newcommand{\facrefss}[4][and]{Facts~\ref{fac:#2}, \ref{fac:#3} #1~\ref{fac:#4}}
\newcommand{\itemrefss}[4][and]{Items~\ref{item:#2}, \ref{item:#3} #1~\ref{item:#4}}
% References to four items at a time
%\newcommand{\eqrefsss}[5][and]{Equations~\ref{eq:#2}, \ref{eq:#3}, \ref{eq:#4} #1~\ref{eq:#5}}
\newcommand{\eqrefsss}[5][and]{(\ref{eq:#2}), (\ref{eq:#3}), (\ref{eq:#4}) #1~(\ref{eq:#5})}
\newcommand{\secrefsss}[5][and]{Sections~\ref{sec:#2}, \ref{sec:#3}, \ref{sec:#4} #1~\ref{sec:#5}}
\newcommand{\apprefsss}[5][and]{Appendices~\ref{app:#2}, \ref{app:#3}, \ref{app:#4} #1~\ref{app:#5}}
\newcommand{\figrefsss}[5][and]{Figures~\ref{fig:#2}, \ref{fig:#3}, \ref{fig:#4} #1~\ref{fig:#5}}
\newcommand{\tabrefsss}[5][and]{Tables~\ref{tab:#2}, \ref{tab:#3}, \ref{tab:#4} #1~\ref{tab:#5}}
\newcommand{\algrefsss}[5][and]{Algorithms~\ref{alg:#2}, \ref{alg:#3}, \ref{alg:#4} #1~\ref{alg:#5}}
\newcommand{\thmrefsss}[5][and]{Theorems~\ref{thm:#2}, \ref{thm:#3}, \ref{thm:#4} #1~\ref{thm:#5}}
\newcommand{\lemrefsss}[5][and]{Lemmas~\ref{lem:#2}, \ref{lem:#3}, \ref{lem:#4} #1~\ref{lem:#5}}
\newcommand{\correfsss}[5][and]{Corollaries~\ref{cor:#2}, \ref{cor:#3}, \ref{cor:#4} #1~\ref{cor:#5}}
\newcommand{\defrefsss}[5][and]{Definitions~\ref{def:#2}, \ref{def:#3}, \ref{def:#4} #1~\ref{def:#5}}
\newcommand{\facrefsss}[5][and]{Facts~\ref{fac:#2}, \ref{fac:#3}, \ref{fac:#4} #1~\ref{fac:#5}}
\newcommand{\itemrefsss}[5][and]{Items~\ref{item:#2}, \ref{item:#3}, \ref{item:#4} #1~\ref{item:#5}}

% Theorem environments.
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}

% Paragraph environment with a leading boldface title.
\newenvironment{titled-paragraph}[1]{\textbf{#1:}}{}

% some named thingies (non-mathmode)
\newcommand{\matlab}{MATLAB\xspace}
\newcommand{\cplusplus}{C++\xspace}
\newcommand{\tensorflow}{TensorFlow\xspace}
\newcommand{\nullptr}{\emph{null}\xspace}
\newcommand{\etal}{et~al.\xspace}
\newcommand{\iid}{\emph{i.i.d.}\xspace}
\newcommand{\wrt}{w.r.t.\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\eg}{e.g.\xspace}
\newcommand{\egcite}[1]{\citep[\eg][]{#1}}

% probability, expectation, variance indicator (mathmode)
%\newcommand{\probability}{\ensuremath{\mathbb{P}}}
\newcommand{\probability}{\ensuremath{P}}
\newcommand{\expectation}{\ensuremath{\mathbb{E}}}
\newcommand{\variance}{\ensuremath{\mathrm{Var}}}
\newcommand{\indicator}{\ensuremath{\mathbb{I}}}

% some operators
\newcommand{\defeq}{\ensuremath{\vcentcolon=}}
\newcommand{\eqdef}{\ensuremath{=\vcentcolon}}
\newcommand{\symdif}{\ensuremath{\triangle}}

% complex, natural, rational, real, integer numbers (mathmode)
%\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}

% for optimization problems (mathmode)
\newcommand{\minimize}[1][]{\ensuremath{\underset{#1}{\mathrm{minimize}}\;}}
\newcommand{\maximize}[1][]{\ensuremath{\underset{#1}{\mathrm{maximize}}\;}}
\newcommand{\suchthat}[1][]{\ensuremath{\underset{#1}{\mathrm{s.t.}}\;}}
\newcommand{\where}{\ensuremath{\mathrm{where}\;}}

% extra math stuff (mathmode)
\newcommand{\inner}[2]{\ensuremath{\left\langle {#1}, {#2} \right\rangle}\xspace}
\newcommand{\bra}[1]{\ensuremath{\left\langle {#1} \right\vert}\xspace}
\newcommand{\ket}[1]{\ensuremath{\left\vert {#1} \right\rangle}\xspace}
\newcommand{\norm}[1]{\ensuremath{\left\lVert {#1} \right\rVert}\xspace}
\newcommand{\lnorm}[1]{\ensuremath{\left\lVert {#1} \right.}\xspace}
\newcommand{\rnorm}[1]{\ensuremath{\left. {#1} \right\rVert}\xspace}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil {#1} \right\rceil}\xspace}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor {#1} \right\rfloor}\xspace}
\newcommand{\abs}[1]{\ensuremath{\left\lvert {#1} \right\rvert}\xspace}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

% extra set stuff (mathmode)
\newcommand{\indices}[1]{\ensuremath{\left[#1\right]}}
%\newcommand{\indices}[1]{\ensuremath{\left\{1,2,\dots,#1\right\}}}
\newcommand{\powerset}[1]{\ensuremath{\mathcal{P}(#1)}}
%\newcommand{\powerset}[1]{\ensuremath{2^{#1}}}
\newcommand{\cardinality}[1]{\ensuremath{\abs{#1}}}

% extra matrix stuff (mathmode)
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag}

% domain and range
\DeclareMathOperator{\domain}{domain}
\DeclareMathOperator{\range}{range}

% pseudocode
\newcommand{\code}[1]{\mbox{\texttt{#1}}}
\newcommand{\codecomment}[1]{\`//~\textit{#1}}
\newcounter{lineno}
\newenvironment{pseudocode}{\setcounter{lineno}{0}\begin{tabbing}\textbf{mm}\=mm\=mm\=mm\=mm\=\kill}{\end{tabbing}}
\newcommand{\codename}{\>}
\newcommand{\codecommentline}[1]{\>\stepcounter{lineno}\textbf{\arabic{lineno}}\'\>//~\textit{#1}}
\newcommand{\codeline}{\>\stepcounter{lineno}\textbf{\arabic{lineno}}\'\>}
\newcommand{\codeskip}{\>\>}

% Notation unique to this paper

% Class-dependent pairwise accuracy
\newcommand{\pacc}[2]{\ensuremath{A_{#1>#2}}}
\newcommand{\cacc}[1]{\ensuremath{A_{#1}}}

% Group matrix.
\newcommand{\M}{\mathbb{M}}

% Group pairs.
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\cS}{\mathcal{S}}
%%

\newcommand{\1}{\mathbf{1}}
\newcommand{\hlgt}[1]{{\color{blue} #1}}
\newcommand{\cL}{\mathcal{L}}

